Time- and Communication-Efficient Overlay Network Construction via Gossip

We focus on the well-studied problem of distributed overlay network construction. We consider a synchronous gossip-based communication model where in each round a node can send a message of small size to another node whose identifier it knows. The network is assumed to be reconfigurable, i.e., a node can add new connections (edges) to other nodes whose identifier it knows or drop existing connections. Each node initially has only knowledge of its own identifier and the identifiers of its neighbors. The overlay construction problem is, given an arbitrary (connected) graph, to reconfigure it to obtain a bounded-degree expander graph as efficiently as possible. The overlay construction problem is relevant to building real-world peer-to-peer network topologies that have desirable properties such as low diameter, high conductance, robustness to adversarial deletions, etc. Our main result is that we show that starting from any arbitrary (connected) graph $G$ on $n$ nodes and $m$ edges, we can construct an overlay network that is a constant-degree expander in polylog $n$ rounds using only $\tilde{O}(n)$ messages. Our time and message bounds are both essentially optimal (up to polylogarithmic factors). Our distributed overlay construction protocol is very lightweight as it uses gossip (each node communicates with only one neighbor in each round) and also scalable as it uses only $\tilde{O}(n)$ messages, which is sublinear in $m$ (even when $m$ is moderately dense). To the best of our knowledge, this is the first result that achieves overlay network construction in polylog $n$ rounds and $o(m)$ messages. Our protocol uses graph sketches in a novel way to construct an expander overlay that is both time and communication efficient. A consequence of our overlay construction protocol is that distributed computation can be performed very efficiently in this model.

==> figure.tex <==

\begin{figure}[H]
     \centering
     \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[page=2,width=0.8\linewidth]{figures/pics.pdf}
        \caption{}
        \label{fig:step-onea}
     \end{subfigure} \hfill
     \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[page=3,width=0.8\linewidth]{figures/pics.pdf}
        \caption{}
        \label{fig:step-oneb}
     \end{subfigure} \vspace{0.2cm}

     \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[page=4,width=0.8\linewidth]{figures/pics.pdf}
        \caption{}
        \label{fig:step-onec}
     \end{subfigure} \hfill
     \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[page=5,width=0.8\linewidth]{figures/pics.pdf}
        \caption{}
        \label{fig:step-oned}
     \end{subfigure} \vspace{0.2cm}

     \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[page=6,width=0.8\linewidth]{figures/pics.pdf}
        \caption{}
        \label{fig:step-onee}
     \end{subfigure} \hfill
     \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[page=7,width=0.8\linewidth]{figures/pics.pdf}
        \caption{}
        \label{fig:step-onef}
     \end{subfigure}
     
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[page=8,width=0.8\linewidth]{figures/pics.pdf}
        \caption{}
        \label{fig:step-oneg}
     \end{subfigure} \hfill
\caption{Figures illustrating three rounds of step one run on a cluster of $10$ nodes. In each round, each node chooses at most two of its neighbors (indicated by arrows) to send messages to. Each node then keeps track of the smallest ID's message it has seen so far. Notice how two nodes that have the same minimum ID (Blue) can be disconnected from one another in the middle of the protocol. However, by the end of the protocol, all nodes within a given cluster should be aware of exactly one minimum ID with high probability.}
\label{fig:step-one}
\end{figure}
